Learning Hierarchical Relational Representations through Relational Convolutions

An evolving area of research in deep learning is the study of architectures and inductive biases that support the learning of relational feature representations. In this paper, we address the challenge of learning representations of hierarchical relations--that is, higher-order relational patterns among groups of objects. We introduce "relational convolutional networks", a neural architecture equipped with computational mechanisms that capture progressively more complex relational features through the composition of simple modules. A key component of this framework is a novel operation that captures relational patterns in groups of objects by convolving graphlet filters--learnable templates of relational patterns--against subsets of the input. Composing relational convolutions gives rise to a deep architecture that learns representations of higher-order, hierarchical relations. We present the motivation and details of the architecture, together with a set of experiments to demonstrate how relational convolutional networks can provide an effective framework for modeling relational tasks that have hierarchical structure.

==> experiments_set_old.tex <==
\subsection{\textit{Set}: Grouping and Compositionality in Relational Reasoning}\label{ssec:experiments_set}

\textit{Set} is a card game that forms a simple but challenging relational task. The `objects' are a set of cards with four attributes, each of which can take one of three possible values. `Color' can be red, green, or purple; `number' can be one, two, or three; `shape' can be diamond, squiggle, or oval; and `fill' can be solid, striped, or empty. A `set' is a triplet of cards such that each attribute is either a) the same on all three cards, or b) different on all three cards.

\begin{figure}[ht]
    \vskip-10pt
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \raisebox{20pt}{\includegraphics[width=\textwidth]{figs/contains_set_example.pdf}}
        \caption{Example of ``contains set'' task.}\label{fig:contains_set_example}
    \end{subfigure}
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/experiments/contains_set_acc.pdf}
        \vskip-5pt
        \caption{\footnotesize{Hold-out test accuracy.}}\label{fig:contains_set_acc}
    \end{subfigure}

    \begin{subfigure}[t]{0.97\textwidth}
        \centering
        \includegraphics[width=0.975\textwidth]{figs/experiments/contains_set_training_curves.pdf}
        \caption{Training accuracy and validation accuracy over the course of training.}\label{fig:contains_set_training_curves}
    \end{subfigure}
    % \begin{subfigure}[t]{0.45\textwidth}
    %     \centering
    %     \includegraphics[width=0.9\textwidth]{figs/experiments/contains_set_training_curves_trainacc.pdf}
    %     \vskip-5pt
    %     \caption{Training accuracy over the course of training.}\label{fig:contains_set_training_curves_trainacc}
    % \end{subfigure}
    % \begin{subfigure}[t]{0.45\textwidth}
    %     \centering
    %     \includegraphics[width=0.9\textwidth]{figs/experiments/contains_set_training_curves_valacc.pdf}
    %     \vskip-5pt
    %     \caption{Validation accuracy over the course of training.}\label{fig:contains_set_training_curves_valacc}
    % \end{subfigure}
    \caption{Results of ``contains set'' experiments. Bar height/solid lines indicate the mean over 10 trials and error bars/shaded regions indicate 95\% bootstrap confidence intervals.}\label{fig:contains_set_experiment}
    \vskip-5pt
\end{figure}

% \begin{figure}[ht]
%     \centering
%     \begin{minipage}{0.49\textwidth}
%         \includegraphics[width=0.9\textwidth]{figs/contains_set_example.pdf}
%         \caption{Example of the ``contains set'' task.}\label{fig:contains_set_example}
%     \end{minipage}
%     \begin{minipage}{0.49\textwidth}
%         \includegraphics[width=0.9\textwidth]{figs/experiments/contains_set_acc.pdf}
%         \caption{Hold-out test accuracy. Bar height indicates mean over 10 trials and error bars indicate 95\% confidence intervals.}\label{fig:contains_set_acc}    
%     \end{minipage}
% \end{figure}

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.4\textwidth]{figs/contains_set_example.pdf}
%     \vskip-12pt
%     \caption{Example of the ``contains set'' task.}\label{fig:contains_set_example}
%     \vskip-7pt
% \end{figure}

In \textit{Set}, the task is: given a hand of $n > 3$ cards, find a `set' among them.~\Cref{fig:contains_set_example} depicts a positive and negative example for $n=5$, with $*$ indicating the `set' in the positive example.
% (typically, \textit{Set} is played with $k=12$, with two players competing to find a `set' first). 
This task is deceptively challenging, and is representative of the type of relational reasoning that humans excel at but machine learning systems still struggle with. To solve the task, one must process the sensory information of individual cards to identify the values of each attribute, and then reason about the relational pattern in each triplet of cards.
% Importantly, this type of relational reasoning requires attending over several attributes and relations simultaneously while representing some notion of `groups'.  
The construct of relational convolutions proposed in this paper is a step towards developing machine learning systems that can perform this kind of relational reasoning.

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.4\textwidth]{figs/experiments/contains_set_acc.pdf}
%     % \vskip-12pt
%     \caption{Hold-out test accuracy. Bar height indicates mean over 10 trials and error bars indicate 95\% confidence intervals.}\label{fig:contains_set_acc}
%     % \vskip-10pt
% \end{figure}

In this section, we evaluate RelConvNet on a task based on \textit{Set} and compare it to several baselines. The task is: given a collection of $n=5$ images of \textit{Set} cards, determine whether or not they contain a `set'. All models share the common architecture $(x_1, \ldots, x_n) \to \texttt{CNN} \to \{ \cdot \} \to \texttt{MLP} \to \hat{y}$, where $\{\cdot\}$ indicates the central module being tested. In addition to CoRelNet, PrediNet, and Transformers, we also compare RelConvNet to several GNN baselines. The CNN embedder is pre-trained on the task of classifying the four attributes of the cards and an intermediate layer is used to generate embeddings. The output MLP architecture is shared across all models.
%  of dimension $64$ for each card. The output MLP architecture is shared across all models, and consists of two hidden layers with $64$ and $32$ neurons, respectively, and ReLU activations. 
Further architectural details can be found in~\Cref{sec:experiments_supplement}. 

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.8\textwidth]{figs/experiments/contains_set_training_curves.pdf}
%     % \vskip-10pt
%     \caption{Training accuracy and validation accuracy over the course of training. Solid lines indicate mean over 10 trials and shaded regions indicates 95\% bootstrap confidence intervals.}\label{fig:contains_set_training_curves}
%     % \vskip-12pt
% \end{figure}

In \textit{Set}, there exists $\binom{81}{3} = 85\,320$ triplets of cards, of which $1\,080$ are a `set'. We partition the `sets' into training (70\%), validation (15\%), and test (15\%) sets. The training, validation, and test datasets are generated by sampling $k$-tuples of cards such that with probability $1/2$ the $k$-tuple does not contain a set, and with probability $1/2$ it contains a set among the corresponding partition of sets. Partitioning the data in this way allows us to measure the models' ability to ``learn the rule'' and identify new unseen `sets'.
We train for 100 epochs with the same loss, optimizer, and batch size as the experiments in the previous section. For each model, we run 10 trials with different random seeds.
\Cref{fig:contains_set_acc} shows the hold-out test accuracy for each model.~\Cref{fig:contains_set_training_curves} shows the training and validation accuracy over the course of training.

We observe a sharp separation between RelConvNet and all other baselines. While RelConvNet is able to learn the task and generalize to new `sets' with near-perfect accuracy (avg: 97.9\%), no other model is able to reach generalization accuracy much better than random guessing (next best is the LSTM with 60.2\%). Several models are able to fit the training data, reaching near-perfect training accuracy, but they are unable to ``learn the rule'' in a way that generalizes to the validation or test sets. This suggests that while these models are powerful function approximators, they lack the \textit{inductive biases} to learn hierarchical relations.

%\aanote{this part is new.}
In~\Cref{fig:conv_rep} we analyze the geometry of the representations learned by the relational convolution layer. We consider all triplets of cards, compute the relation subtensor using the learned MD-IPR layer, and plot the relational inner product with the learned graphlet filter $\bm{f} \in \reals^{s \times s \times d_r \times n_f}$. The result is a $n_f$-dimensional vector for each triplet of cards. We perform PCA to plot this in two dimensions, and color-code each triplet of cards according to whether or not it forms a `set'. We find that the relational convolution layer learns a representation of the relational pattern in groups of objects that separates `sets' and `non-sets'. In particular, the two classes form clusters that are linearly separable even when projected down to two dimensions by PCA. This explains why RelConvNet is able to learn the task in a way that generalizes while the other models are not. In~\Cref{sec:appendix_rep_analysis} we expand on this discussion, and further analyze the representations learned by the MD-IPR layer, showing that the learned relations map to the color, number, shape, and fill attributes.

\begin{wrapfigure}{R}{0.5\textwidth}
    \centering
    \includegraphics[width=0.5\textwidth]{figs/representation_analysis/conv_rep.pdf}
    \caption{The relational convolution layer produces representations that separates `sets' from `non-sets'.}\label{fig:conv_rep}
\end{wrapfigure}

It is perhaps surprising that models like GNNs and Transformers perform poorly on these relational tasks, given their apparent ability to process relations through neural message-passing and attention, respectively. We remark that GNNs operate in a different domain compared to relational models like RelConvNe, PrediNet, and CoRelNet. In GNNs, the relations are an input to the model, received in the form of a graph, and are used to dictate the flow of information in a neural message-passing operation. By contrast, in relational convolutional networks, the input is simply a set of objects without relations---the relations need to be \textit{inferred} as part of the feature representation process. 
Thus, GNNs operate in domains where relational information is already present (e.g., analysis of social networks, biological networks, etc.), whereas our framework aims to solve tasks that rely on relations but those relations need to be inferred end-to-end. 
This offers a partial explanation for the inability of GNNs to learn this task---GNNs are good at processing network-style relations when they are given as input, but may not be able to infer and hierarchically process relations when they are not given. In the case of Transformers, relations are modeled implicitly to direct information retrieval in attention, but are not encoded explicitly in the final representations. By contrast, RelConvNet operates on collections of objects and possesses inductive biases for learning iteratively more complex relational representations, guided only by the supervisory signal of the downstream task. 

Models like CoRelNet and PrediNet have relational inductive biases, but lack compositionality. On the other hand, deep models like Transformers and GNNs are compositional, but lack relational inductive biases. This experiment suggests that \textit{compositionality and relational inductive biases are both necessary ingredients to efficiently learn representations of higher-order relations}. RelConvNet is a compositional architecture imbued with relational inductive biases and a demonstrated ability to tackle hierarchical relational tasks.


==> figs/experiments/relgames_group_architectures_table.tex <==
\begin{tabular}{p{0.25\textwidth}p{0.75\textwidth}}
    \toprule
    Grouping layer & Description \\\hline
    Temporal Grouping & $G$ learned directly as parameter.\\\hline
    Feature-based Grouping & $G$ produced by MLP with two hidden layers of size 32 and relu activation. \\\hline
    Contextual Grouping & $G$ produced by message-passing (via Transformer Encoder Block) followed by an MLP (\cref{eq:context_grouping}). Encoder Block has 4 heads, inner dim = 32, and relu activation. MLP same as feature-based grouping.\\
    \bottomrule
\end{tabular}

==> grouping_layers.tex <==
\section{Grouping Layers}\label{sec:grouping_layers}

\textcolor{red}{remove this section if we use the alternate `soft groups' model.}

A grouping layer is a layer which outputs a group matrix $G \in \reals^{m \times n_g}$ representing the degree to which each object $i \in [m]$ belongs to each group $j \in [n_g]$. The number of groups $n_g$ is a configurable hyperparameter. We briefly describe some proposals for grouping layers with different properties.

\textbf{Temporal (Positional) Grouping.} In the temporal grouping layer, the groups are a function only of the temporal order of the objects. This can be achieved by learning the group matrix $G$ directly as a parameter of the model. $G$ will be optimized along with the rest of the model parameters as a function of its effect on the relational convolution layer. Temporal grouping would be appropriate in situations where the order in which objects appear is predetermined and indicates the relevant groups. For example, objects that are positionally close to each other may be grouped together.

\textbf{Feature-based Grouping.} In a feature-based grouping layer, the group(s) to which each object belongs is a function of that object's features (and position). That is,
\begin{equation}\label{eq:feat_grouping}
        G \gets \begin{bmatrix}
            \phi(1, x_1)^\top \\
            \vdots \\
            \phi(m, x_m)^\top
        \end{bmatrix} \in \reals^{m \times n_g},
\end{equation}

\noindent where $\phi: [m] \times \calX \to \reals^{n_g}$ is a learnable function which maps an object's temporal order $i$ and feature representation $x_i$ to a $n_g$-dimensional group membership vector where the $j$th entry of the vector represents the degree to which the object belongs to the $j$th group. For example $\phi$ can be a multi-layer perceptron of the form $\phi(i, x) = \mathrm{MLP}(\mathrm{concat}(e_i, x))$. Feature-based grouping may be useful in situations where group membership can be determined for each object using only that object's features, irrespective of the context of the other objects in the sequence.

\textbf{Context-aware Grouping.} In some applications, the group(s) to which each object belongs to may depend on the full context of the other objects in the sequence. One way to model this is to use a message-passing neural network to update the representations of each object, incorporating the context of the other objects in the sequence. Then, a multi-layer perceptron is applied to each encoded object to produce the group membership vector for that object.
\begin{equation}\label{eq:context_grouping}
    \begin{split}
        E_i &\gets \mathrm{MessagePassing}\paren{x_i, \set{x_1, \ldots, x_m}}, \ i \in [m] \\
        G &\gets \begin{bmatrix}\mathrm{MLP}(E_1)^\top \\ \vdots \\ \mathrm{MLP}(E_m)^\top \end{bmatrix} \in \reals^{m \times n_g}.
    \end{split}
\end{equation}

This is the most general form of grouping, as it encompasses the previous two forms as special cases. The updated representation of each object $E_i$ now contains any relevant information about the other objects which should be considered in computing its group membership vector. One simple and effective option for the message-passing operation is to use self-attention. In this case, since an inner product relation layer precedes the relational convolution layer, the relation tensor can be re-used in the self-attention operation to compute attention scores.

==> mhr_univ_approx.tex <==
\awni{todo---post to arxiv and add citation. Also, is statement as a theorem necessary, or should we just state the result in text?}

\citep{arxivInnerprodUnivApprox} analyzes the function class of relation functions on $\calX \times \calX$ realizable by inner products of neural network transformations of the form $\iprod{\phi(x)}{\psi(y)}$. The result implies that when $\phi_i, \psi_i$ are multi-layer perceptrons, $r(x,y)$ in~\Cref{eq:relation_function} can approximate any continuous function from $\calX \times \calX$ to $\reals^{d_r}$ uniformly and with arbitrary precision, provided that $\calX$ is a compact subset of euclidean space.

\begin{theorem}[Theorem 3.1 in~\citep{arxivInnerprodUnivApprox}]
    Suppose $\calX$ is a compact subset of euclidean space. Consider the relation model,
    \begin{equation*}
        \hat{r}(x, y) := \paren{\iprod{\phi_\theta^{(1)}(x)}{\psi_\theta^{(1)}(y)}, \ldots, \iprod{\phi_\theta^{(d_r)}(x)}{\psi_\theta^{(d_r)}(y)}},
    \end{equation*}
    \noindent where $\phi_\theta^{(i)}, \psi_\theta^{(i)}: \calX \to \reals^d$ are multi-layer perceptrons with parameters in $\theta$. Then, for any continuous relation function $r: \calX \times \calX \to \reals^{d_r}$ there exists multi-layer perceptrons with parameters $\theta$ such that $\hat{r}$ approximates $r$ uniformly over $(x,y) \in \calX \times \calX$. Formally, for any $\epsilon > 0$, there exists neural networks with parameters $\theta$ such that,
    \begin{equation*}
        \sup_{x, y \in \calX} \infnorm{r(x,y) - \hat{r}(x,y)} < \epsilon.
    \end{equation*}
\end{theorem}

==> old_rel_conv_softgroups.tex <==
% THIS IS THE OLD PROPOSAL OF RELATIONAL CONVOLUTIONS WITH LEARNED SOFT GROUPS
% THE EXPERIMENTS WITH THIS WERE PROMISING, BUT IT IS COMPUTATIONALLY TOO EXPENSIVE
% DUE TO THE NEED TO COMPUTE RELCONV WITH ALL DISCRETE GROUPS AS AN INTERMEDIATE STEP.
% THE NEW PROPOSAL OF "GROUP ATTENTION" IS MORE ELEGANT AND COMPUTATIONALLY EFFICIENT.
% THIS IS THE OLD PROPOSAL, FOR REFERENCE.

\subsection{Relational convolutions with `soft' groups}

In the above formulation, the groups are `discrete'. Having discrete groups can be desirable for interpretability, if the relevant groupings are known a priori or if considering every possible grouping is computationally and statistically feasible. However, if the relevant groupings are not known, then considering all possible combinations results in a rapid growth of the number of objects at each layer.
% Besides being computationally intractable, considering every possible grouping may be unnecessary and may make learning more difficult.

In order to address these issues, we propose \textit{explicitly modeling groups}. This allows us to control the number of objects in the output sequence of a relational convolution operation such that only relevant groups are considered. In the next section, we outline some ways to model `soft groups' using \textit{grouping layers}. These layers take a sequence of objects and/or the relation tensor as input and produce a `group matrix' $G \in \reals^{n \times n_g}$ representing $n_g$ `soft groups'. The $(i,j)$-th entry of the group matrix represents the degree to which the $i$-th object belongs to the $j$-th group. The number of groups $n_g$ is a configurable hyperparameter of the grouping layers. For the remainder of this subsection, we assume that the group matrix $G$ is given as input to the relational convolution layer.

Consider the group matrix $G \in \reals^{n \times n_g}$ and filters $\bm{f}$ of size $s$. First, we use $G$ to compute a ``group-match score'' for each discrete group $g$ of size $s$ (e.g., $g \in \calG = \binom{[n]}{s}$). This is done via
\begin{equation}\label{eq:group_match_score}
    \begin{split}
        G &\gets \text{SoftPlus}(G)\\
        \alpha_{gk} &\gets \text{Normalize}\paren{\bra{\prod_{i \in g} G[i,k]}_{g \in \calG}}, \quad g \in \calG, k \in [n_g],
    \end{split}
\end{equation}
where the soft-plus function is $\text{Softplus}(x) = \log(\exp(x + 1))$, applied elementwise. This has the effect of making the group matrix $G$ non-negative which is needed for the product of its elements to represent a ``group-match score''. The product inside the softmax is over elements in the discrete group $g \in \calG$. Hence, it will be large whenever the soft group $G_k := G[:, k]$ aligns with the discrete group $g$. $\mathrm{Normalize}(\cdot)$ normalizes the group match scores so that $\sum_{g} \alpha_{gk} = 1$. We propose the use of sparse normalizers~\citep{lahaControllableSparseAlternatives2018a} so that only a sparse subset of discrete groups in $\calG$ contribute to each soft group (see also~\Cref{ssec:computational_considerations}). In our experiments, we use `sparsemax'~\citep{martinsSoftmaxSparsemaxSparse2016}. Thus, $\alpha_{gk}$ is a normalized ``group-match score'' indicating the degree to which the discrete group $g$ matches the given soft group $G_k$.
% \footnote{Sparse normalizers would likely be appropriate alternatives to softmax here, since it would be desirable to have only a sparse subset of discrete groups in $\calG$ contribute to each soft group. Some sparse alternatives to softmax are discussed in~\citep{lahaControllableSparseAlternatives2018a}.}. %Note that the group match scores of discrete groups sum to one, $\sum_{g \in G} \alpha_{gk} = 1, \ \forall k \in [n_g]$.

Now, we can define the `soft' relational inner product \textit{given} the soft group $G_k$ by
\begin{equation}\label{eq:soft_relational_inner_prod}
    \langle R, \boldsymbol{f} \, \vert \, G_k \rangle_R \coloneqq \sum_{g \in \calG} \alpha_{gk} \iprod{R[g]}{\boldsymbol{f}}_\mathrm{rel}.
\end{equation}
This notation should be read as ``the relational inner product of the relation tensor $R$ with the graphlet filters $\boldsymbol{f}$ given the group $G_k$''. This expression is essentially a convex combination of the relational inner product with all possible discrete groups weighted by how much they match the soft group $G_k$.

With this modification, the number of objects in the output sequence is fixed and controlled by the number of groups, $n_g$ (which is a hyperparameter). The output sequence of the relational convolution given groups $G$ is now given by
\begin{equation}\label{eq:soft_relational_convolution_groups}
    (R \ast \bm{f})(G) = \left( \softreliprod{R}{\bm{f}}{G_1}, \ldots, \softreliprod{R}{\bm{f}}{G_{n_g}} \right) \in \left(\mathbb{R}^{n_f}\right)^{n_g}.
\end{equation}


==> related_work.tex <==
\subsection{Related Work}

Several previous works have considered the design of machine learning architectures which support the representation of relational information in various forms~\citep{battagliaRelationalInductiveBiases2018}%,palmRecurrentRelationalNetworks2018,zhangRAVENDatasetRelational2019}. % battaglia is a review of "relational inductive biases" (though in a somewhat different sense to us). the rest are more specific, so this may not be the best place to cite them.

\textbf{Graph Neural Networks.} Graph neural networks (GNNs) are a class of neural network architectures which operate on graphs and process ``relational'' data~\citep{niepertLearningConvolutionalNeural2016,kipfSemiSupervisedClassificationGraph2017,schlichtkrullModelingRelationalData2017,velickovicGraphAttentionNetworks2017,kipfNeuralRelationalInference2018,xuHowPowerfulAre2018}. A defining feature of the GNN model is its use of a form of neural message-passing, wherein the hidden representation of a node is updated as a function of the hidden representations of its neighbors on a graph~\citep{gilmerNeuralMessagePassing2017}. Typical examples of tasks which GNNs are applied to include node classification, graph classification, and link prediction~\citep{hamiltonGraphRepresentationLearning2020}. %This is a very general model which includes as a special case convolutional neural networks, where the graph is a grid, and Transformers, where the graph is a complete graph and the message-passing function is a convex sum of the neighbors' representations. In our experiments, we compare to Transformers as a representative of the GNN model.

In GNNs, the `relations' are given to the model via edges in a graph. In contrast, our architecture, as well as the explicitly relational architectures described below, operate on collections of objects without any relations given as input. Instead, such relational architectures must infer the relevant relations from the objects themselves. Still, graph neural networks can be applied to relational tasks by passing in the collection of objects along with a complete graph. % A Transformer Encoder can be thought of as a special case of this architecture.%, and hence is the representative baseline we compare against in our experiments.

\textbf{Attention as modeling relations} Several works have proposed architectures with the ability to model relations by incorporating an attention mechanism~\citep{vaswani2017attention,locatelloObjectCentricLearningSlot2020,santoroRelationalRecurrent2018,zambaldiDeepReinforcementLearning2018,velickovicGraphAttentionNetworks2017}. Attention mechanisms, such as self-attention in Transformers~\citep{vaswani2017attention}, model relations between objects implicitly as an intermediate step in a form of neural message-passing in order to update the representation of each object as a function of its context.

\textbf{Emerging literature on ``explicitly relational'' architectures.} There exists a growing literature on neural architectures which aim to explicitly model relational information between objects. An early example is the relation network proposed by~\citet{santoroSimpleNeural2017}.~\citet{shanahanExplicitlyRelationalNeural} proposes the PrediNet architecture, which aims to learn relational representations which are compatible with predicate logic.~\citet{webbEmergentSymbols2021} proposes ESBN, a recurrent neural network augmented with external memory whose memory-write operation aims to factors representations into `sensory' and `relational'.~\citet{kergNeuralArchitecture2022} proposes CoRelNet, a simple architecture based on `similarity scores' which aims to distill the relational inductive biases discovered in previous work into a minimal architecture.~\citet{altabaaAbstractorsRelationalCrossattention2024} explored relational inductive biases in the context of Transformers, and proposed a view of relational inductive biases as a type of selective ``information bottleneck'' which disentangles relational information from object-level features.~\citet{webbRelationalBottleneckInductive2023} provides a cognitive science perspective on this idea, arguing that a relational information bottleneck may be a mechanism for abstraction in the human mind.% and brain.

In this paper, we contribute relational convolutional networks to this literature. What sets relational convolutional networks apart from existing relational architectures is its  compositionality and its ability to learn higher-order relations.

